Correlation-Guided Query-Dependency Calibration for Video Temporal Grounding

Temporal Grounding is to identify specific moments or highlights from a video corresponding to textual descriptions. Typical approaches in temporal grounding treat all video clips equally during the encoding process regardless of their semantic relevance with the text query. Therefore, we propose Correlation-Guided DEtection TRansformer (CG-DETR), exploring to provide clues for query-associated video clips within the cross-modal attention. First, we design an adaptive cross-attention with dummy tokens. Dummy tokens conditioned by text query take portions of the attention weights, preventing irrelevant video clips from being represented by the text query. Yet, not all words equally inherit the text query's correlation to video clips. Thus, we further guide the cross-attention map by inferring the fine-grained correlation between video clips and words. We enable this by learning a joint embedding space for high-level concepts, i.e., moment and sentence level, and inferring the clip-word correlation. Lastly, we exploit the moment-specific characteristics and combine them with the context of each video to form a moment-adaptive saliency detector. By exploiting the degrees of text engagement in each video clip, it precisely measures the highlightness of each clip. CG-DETR achieves state-of-the-art results on various benchmarks for temporal grounding. Codes are available at https://github.com/wjun0830/CGDETR.

==> figure/figure_5.tex <==
\begin{figure*}[t!]
    \centering
    \vspace{-0.2cm}
    \includegraphics[width=0.97\textwidth]{figure/fig_6.pdf}
    \vspace{-0.25cm}
    \caption{Visualization of prediction comparisons on QVHighlights.}
    \vspace{-0.6cm}
    \label{fig:qualitative_main}
\end{figure*}


==> figure/figure_word_attn.tex <==
\begin{figure}[t!]
    \centering
    \vspace{-0.2cm}
    \includegraphics[width=1.0\columnwidth]{figure/fig_7.pdf}
    \vspace{-0.5cm}
    % \includegraphics[width=1.0\columnwidth]{figure/fig_word_attn_supp_test.pdf}
    \caption{
    % Examination of learned correlation between video clips and text query in CG-DETR.
    % % Examination of learned correlation between video clips and text query. 
    % Each row comes from the same example.
    % (Left) Comparison between the degrees of multimodal interaction and GT saliency scores. (Right) Learned correspondence between each word and video clips.
    % \SE{}
    Examination of learned correlation between video clips and query in CG-DETR with two video-text pairs.
    Line graphs plot the comparison between the degrees of multimodal interaction and GT saliency scores, and heatmaps show the learned correspondence between each word and video clip. 
    }
    \label{fig:word_attn}
    \vspace{-0.35cm}
\end{figure}
% \vspace{-0.6cm}

